Asymptotic-Preserving Schemes for Fluid Models of Plasmas

These notes summarize a series of works related to the numerical approximation of plasma fluid problems. We construct so-called 'Asymptotic-Preserving' schemes which are valid for a large range of values (from very small to order unity) of the dimensionless parameters that appear in plasma fluid models. Specifically, we are interested in two parameters, the scaled Debye length which quantifies how close to quasi-neutrality the plasma is, and the scaled cyclotron period, which is inversely proportional to the magnetic field strength. We will largely focus on the ideas, in order to enable the reader to apply these concepts to other situations.

==> Dirichlet_n.tex <==
For a one-dimensional elliptic problem, two-point boundary conditions are required. However, some compatibility conditions are required for the low Mach-number limit to be valid. Otherwise, either some boundary layers are formed, or simply, the scaling is not correct and the problem is far from a low Mach-number regime. 

Let $y_- \in \Gamma_-$. We denote by $X(s;y_-)$ the magnetic field line issued from $y_-$, parametrized by its curvilinear coordinate $s$. $X(s;y_-)$ exits the domain at a conjugate point $y_+ \in \Gamma_+$ and the corresponding value $s_+$ of $s$ is the arclength of the intersection of the magnetic field line with the domain. 

Now, the validity of the drift-fluid limit imposes that 
\begin{eqnarray}
& & \hspace{-1cm}  \nabla_\parallel p(n^\tau) - n^\tau E_\parallel  = O(\tau),      
\label{DL_constraint} 
\end{eqnarray}
(see e.g. (\ref{RIEL2_u_par}) for instance). 
This implies some constraint for the density at two conjugate points $y_-$ and $y_+$. To express this constraint, we introduce the function $h(n)$ such that $h'(n) = p'(n)/n$. We also introduce a function $\phi(x)$ such that 
\begin{eqnarray}
& & \hspace{-1cm}   E_\parallel  = - \nabla_\parallel \phi.       
\label{def_pot_par} 
\end{eqnarray}
Note that $\phi$ exists without any local condition on the vector field $E$ (such as a curl-free condition) and that it is not an electric potential. Indeed, (\ref{def_pot_par}) is only requested for the parallel component. Therefore, $\phi$ is a primitive of $E_\parallel$ locally along a field line. In order to define it globally, a problem arises for closed field or infinite length field lines, because we need to guarantee that $\phi$ returns to its initial value after one loop around a closed field line, or very close to that value after an infinite number of windings in the case of an infinite field line. Therefore, conditions on $E$ along such field lines are requested. These are 
\begin{eqnarray}
& & \hspace{-1cm}   \oint_{C} E_\parallel ds = 0, \quad \mbox{(respectively that} \quad \frac{1}{S} \lim_{S \to \infty} \oint_{C_{-S,S}} E_\parallel ds = 0    \, \mbox{)}, 
\label{int_cond} 
\end{eqnarray}
for all closed magnetic field lines $C$ (respectively for all infinite length field lines $C$, where $C_{-S,S}$ denotes the interval of the field line comprised between the two points of arc-length coordinates $-S$ and $S$ relative to an arbitrary arc-length origin). These conditions can be viewed as restrictive. However, they can be weakened by assuming that the electric field $E$ depends on $\tau$ and has a Taylor expansion \, $E^\tau = E^0 + \tau E^1 + o(\tau)$. \, Then, conditions (\ref{int_cond}) must only apply to $E^0$. Finally, these constraints are an artefact of the isentropic assumption, and are not needed when the full Euler model is used, because the pressure is no longer a local function of the density only, but also of the temperature. With these definitions, we find that (\ref{DL_constraint}) implies that 
\begin{eqnarray}
& & \hspace{-1cm}  h(n^\tau) - \phi  = \psi + O(\tau), \quad \mbox{with} \quad \nabla_\parallel \psi = 0.       
\label{DL_constraint_2} 
\end{eqnarray}
In other words, $h(n^\tau) - \phi$ is, up to an $O(\tau)$ quantity, constant along the magnetic field lines. Consequently, let $y_\pm \in \Gamma_\pm$ be two conjugate points along the same field line. (\ref{DL_constraint_2}) implies:
\begin{eqnarray}
& & \hspace{-1cm}  h(n^\tau)(y_+) -  h(n^\tau)(y_-) = \phi(y_+) - \phi(y_-) + O(\tau).       
\label{DL_constraint_3} 
\end{eqnarray}
This constraint does not depend on any particular choice of $\psi$: $\psi$ being constant along the field lines, the difference of its values at the two conjugte points is equal to zero. In the small $\tau$ regime, (\ref{DL_constraint_3}) links the values of $n^\tau$ at the conjugate points of magnetic field lines which intersect the boundary. If the magnetic field line is tangent to the boundary, the value of $n$ is constrained all along the boundary by:  
\begin{eqnarray}
& & \hspace{-1cm}  h(n^\tau)(X(s;y_-)) -  h(n^\tau)(y_-) = \phi(X(s;y_-)) - \phi(y_-) + O(\tau), \quad \forall s \in [0,s_+].       
\label{DL_constraint_4} 
\end{eqnarray}

We are now ready to set up the boundary conditions. We assume Dirichlet boundary conditions for the density $n^\tau$ satisfying the constraints (\ref{DL_constraint_3}) and (\ref{DL_constraint_4}): 
\begin{eqnarray}
& & \hspace{-1cm}  n^\tau|_{\Gamma} (y) = n_B^\tau (y), \quad \forall y \in \Gamma,       
\label{IEL_BC_n} 
\end{eqnarray}
with $n_B^\tau$ satisfying (\ref{DL_constraint_3}) and (\ref{DL_constraint_4}). 
